Reachability Games on Extended Vector Addition Systems with States

We consider two-player turn-based games with zero-reachability and zero-safety objectives generated by extended vector addition systems with states. Although the problem of deciding the winner in such games is undecidable in general, we identify several decidable and even tractable subcases of this problem obtained by restricting the number of counters and/or the sets of target configurations.

==> conclusions.tex <==
\section{Conclusions, future work}
\label{sec-concl}

\noindent
Technically, the most involved result presented in this paper is
Theorem~\ref{thm-complexity}. This decidability 
result is not obvious,
%somewhat unexpected,
because most of the problems related to formal verification of Petri
nets (equivalence-checking, model-checking, etc.)  are undecidable
\cite{Esparza:ModelChecking-AI,Jancar:PN-bisimilarity-TCS,%
  JK:EC-Techniques-Results-TPLP,BCMS:Infinite-Structures-HPA}.  Since
the upper complexity bound given in Theorem~\ref{thm-complexity} is
complemented only by the $\EXPSPACE$ lower bound, which is easily
derivable from~\cite{Lipton:PN-Reachability}, there is a
complexity gap which constitutes an interesting challenge for future
work.  We conjecture that for a suitable (and reasonable) choice of
parameters, one might even obtain \emph{fixed parameter tractability}
of the problem. So far, we have not found any arguments against the
hypothesis that the problem is tractable, i.e., solvable in polynomial
time, even for a \emph{fixed number of counters} (note that the
$\EXPSPACE$ lower bound does not hold for a fixed number of counters).



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

